Crosslingual Retrieval Augmented In-context Learning for Bangla

The promise of Large Language Models (LLMs) in Natural Language Processing has often been overshadowed by their limited performance in low-resource languages such as Bangla. To address this, our paper presents a pioneering approach that utilizes cross-lingual retrieval augmented in-context learning. By strategically sourcing semantically similar prompts from high-resource language, we enable multilingual pretrained language models (MPLMs), especially the generative model BLOOMZ, to successfully boost performance on Bangla tasks. Our extensive evaluation highlights that the cross-lingual retrieval augmented prompts bring steady improvements to MPLMs over the zero-shot performance.

==> validation.tex <==
% don't forget that when the prediction doesn't belong to labels, it will be taken as one of the labels: task1-0, task2-negative

\begin{table}[]
\begin{tabular}{|lrrrrrrrr|}
\hline
\multicolumn{1}{|l|}{}                          & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy}       & \multicolumn{1}{c|}{Precision}       & \multicolumn{1}{c|}{Recall}      & \multicolumn{1}{c|}{F1}      \\ \hline
\multicolumn{9}{|l|}{bloomz-3b}                                                                                                                                                                                                                                                                                            \\ \hline
\multicolumn{1}{|l|}{}                          & \multicolumn{4}{c|}{"Does the following sentence represent Direct Violence, Passive Violence, or Non-Violence? \{text\}"} & \multicolumn{4}{c|}{'The nature of the text "\{text\}" is most likely: (Direct Violence, Passive Violence, Non-Violence). Please identify.'} \\ \hline
\multicolumn{1}{|l|}{zero shot}                 & \multicolumn{1}{r|}{48.05}    & \multicolumn{1}{r|}{31.67}     & \multicolumn{1}{r|}{48.05}  & \multicolumn{1}{r|}{28.11} & \multicolumn{1}{r|}{53.76}          & \multicolumn{1}{r|}{47.69}           & \multicolumn{1}{r|}{53.76}       & 30.27                        \\ \hline
\multicolumn{1}{|l|}{bangla-template zero shot} & \multicolumn{1}{r|}{53.91}    & \multicolumn{1}{r|}{29.06}     & \multicolumn{1}{r|}{53.91}  & \multicolumn{1}{r|}{23.35} & \multicolumn{1}{r|}{53.91}          & \multicolumn{1}{r|}{29.06}           & \multicolumn{1}{r|}{53.91}       & 23.35                        \\ \hline
\multicolumn{1}{|l|}{main-1}                    & \multicolumn{1}{r|}{53.23}    & \multicolumn{1}{r|}{32.79}     & \multicolumn{1}{r|}{53.23}  & \multicolumn{1}{r|}{26.01} & \multicolumn{1}{r|}{53.91}          & \multicolumn{1}{r|}{29.06}           & \multicolumn{1}{r|}{53.91}       & 23.35                        \\ \hline
\multicolumn{1}{|l|}{main-3}                    & \multicolumn{1}{r|}{53.38}    & \multicolumn{1}{r|}{32.02}     & \multicolumn{1}{r|}{53.38}  & \multicolumn{1}{r|}{24.47} & \multicolumn{1}{r|}{53.83}          & \multicolumn{1}{r|}{29.07}           & \multicolumn{1}{r|}{53.83}       & 23.34                        \\ \hline
\multicolumn{9}{|l|}{mbert}                                                                                                                                                                                                                                                                                                \\ \hline
\multicolumn{1}{|l|}{}                          & \multicolumn{4}{l|}{{[}MASK{]} violence: \{text\}}                                                                        & \multicolumn{4}{l|}{\{text\} this text is {[}MASK{]} violence.}                                                                              \\ \hline
\multicolumn{1}{|l|}{zero shot}                 & \multicolumn{1}{r|}{36.61}    & \multicolumn{1}{r|}{37.16}     & \multicolumn{1}{r|}{36.61}  & \multicolumn{1}{r|}{30.78} & \multicolumn{1}{r|}{16.54}          & \multicolumn{1}{r|}{86.17}           & \multicolumn{1}{r|}{16.54}       & 11.72                        \\ \hline
\multicolumn{1}{|l|}{main-1}                    & \multicolumn{1}{r|}{40.30}    & \multicolumn{1}{r|}{55.37}     & \multicolumn{1}{r|}{40.30}  & \multicolumn{1}{r|}{25.62} & \multicolumn{1}{r|}{15.78}          & \multicolumn{1}{r|}{93.54}           & \multicolumn{1}{r|}{15.78}       & 10.31                        \\ \hline
\multicolumn{1}{|l|}{main-3}                    & \multicolumn{1}{r|}{40.82}    & \multicolumn{1}{r|}{57.11}     & \multicolumn{1}{r|}{40.82}  & \multicolumn{1}{r|}{25.31} & \multicolumn{1}{r|}{14.81}          & \multicolumn{1}{r|}{98.89}           & \multicolumn{1}{r|}{14.81}       & 8.74                         \\ \hline
\end{tabular}
\caption{results (F1 is macro F1 score) of task1 valid with bloomz-3b and mbert}
\label{tab:results F1 is macro F1 score of task1 valid with bloomz-3b and mbert}
\end{table}


\begin{table}[]
\begin{tabular}{lrrrrrrrrrrrr}
        & \multicolumn{4}{l}{with 1 sample}                                                                                  & \multicolumn{4}{l}{with 3 sample}                                                                                  & \multicolumn{4}{l}{with 5 sample}                                                                                  \\
        & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\
\multicolumn{13}{l}{retrieval similar sample}                                                                                                                                                                                                                                                                                                                          \\
english & 58.13                        & 49.57                         & 58.13                      & 58.13                  & 58.41                        & 49.34                         & 58.41                      & 58.41                  & 57.83                        & 48.71                         & 57.83                      & 57.83                  \\
self    & 58.87                        & 49.94                         & 58.87                      & 58.87                  & 58.52                        & 50.00                         & 58.52                      & 58.52                  & 57.30                        & 49.48                         & 57.30                      & 57.30                  \\
\multicolumn{13}{l}{random sample}                                                                                                                                                                                                                                                                                                                                     \\
english & 56.94                        & 50.00                         & 56.94                      & 56.94                  & 56.66                        & 49.18                         & 56.66                      & 56.66                  & 56.33                        & 48.79                         & 56.33                      & 56.33                  \\
self    & 53.46                        & 49.77                         & 53.46                      & 53.46                  & 53.00                        & 50.41                         & 53.00                      & 53.00                  & 50.03                        & 49.06                         & 50.03                      & 50.03                  \\
\multicolumn{13}{l}{samples per label-retrieval similar sample}                                                                                                                                                                                                                                                                                                        \\
english & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & 57.02                        & 49.35                         & 57.02                      & 57.02                  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   \\
\multicolumn{13}{l}{samples per label-random sample}                                                                                                                                                                                                                                                                                                                   \\
english & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & 55.19                        & 51.07                         & 55.19                      & 55.19                  & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  
\end{tabular}
\caption{results (F1 is micro F1 score) of task2 valid with bloomz-3b model using english and bangla(self, :10000 of train) retrieval dataset, prompt template:"Classify the text as one of the following sentiments:Positive, Negative, or Neutral\textbackslash{}n\textbackslash{}nText:\{text\}\textbackslash{}nSentiment:"}
\label{tab:results F1 is micro F1 score of task2 valid with bloomz-3b model using english and banglaself :10000 of train retrieval dataset}
\end{table}



\begin{table}[]
\begin{tabular}{lrrrrrrrrrrrr}
                                                                                                      & \multicolumn{4}{l}{zero shot}                                                                                      & \multicolumn{4}{l}{with 1 sample}                                                                                  & \multicolumn{4}{l}{with 3 sample}                                                                                  \\
                                                                                                      & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} & \multicolumn{1}{c}{Accuracy} & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c}{F1} \\
pattern 0: \{text\} {[}MASK{]}                                                                        & 23.38                        & 69.49                         & 23.38                      & 23.38                  & 32.02                        & 42.81                         & 32.02                      & 32.02                  & 32.35                        & 42.71                         & 32.35                      & 32.35                  \\
pattern 1: {[}MASK{]}: \{text\}                                                                       & 32.23                        & 48.06                         & 32.23                      & 32.23                  & 36.50                        & 40.22                         & 36.50                      & 36.50                  & 40.08                        & 44.13                         & 40.08                      & 40.08                  \\
pattern 2: {[}MASK{]} text: \{text\}                                                                  & 29.20                        & 51.96                         & 29.20                      & 29.20                  & 37.41                        & 41.00                         & 37.41                      & 37.41                  & 40.82                        & 45.07                         & 40.82                      & 40.82                  \\
pattern 3: \{text\} Sentiment: {[}MASK{]}                                                             & 33.68                        & 44.64                         & 33.68                      & 33.68                  & 38.38                        & 41.48                         & 38.38                      & 38.38                  & 40.87                        & 43.57                         & 40.87                      & 40.87                  \\
pattern 4: \{text\} What is a possible sentiment for the text given the following options: {[}MASK{]} & 38.10                        & 63.58                         & 38.10                      & 38.10                  & 35.23                        & 42.13                         & 35.23                      & 35.23                  & 37.31                        & 40.64                         & 37.31                      & 37.31                  \\
pattern 5: \{text\} Classify the sentiment of this text as Positive, Negative, or Neutral: {[}MASK{]} & 43.69                        & 92.41                         & 43.69                      & 43.69                  & 34.57                        & 40.67                         & 34.57                      & 34.57                  & 37.51                        & 40.07                         & 37.51                      & 37.51                  \\
pattern 6: \{text\} In summary, the sentiment is {[}MASK{]}                                           & 44.38                        & 58.36                         & 44.38                      & 44.38                  & 35.94                        & 42.11                         & 35.94                      & 35.94                  & 38.76                        & 41.21                         & 38.76                      & 38.76                  \\
pattern 7: \{text\} the possible sentiment for the text given the following options is {[}MASK{]}     & 35.46                        & 98.47                         & 35.46                      & 35.46                  & 37.77                        & 42.15                         & 37.77                      & 37.77                  & 40.59                        & 42.06                         & 40.59                      & 40.59                  \\
pattern 8: \{text\} the sentiment of this text as Positive, Negative, or Neutral is {[}MASK{]}        & 43.44                        & 74.14                         & 43.44                      & 43.44                  & 34.79                        & 43.15                         & 34.79                      & 34.79                  & 36.57                        & 41.36                         & 36.57                      & 36.57                  \\
                                                                                                      & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}   & \multicolumn{1}{l}{}         & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{}       & \multicolumn{1}{l}{}  
\end{tabular}
\caption{results of mbert in task2 valid with different templates}
\label{tab:results of mbert in task2 valid with different templates}
\end{table}


\begin{table}[]
\begin{tabular}{|lrrrrrrrrrrrr|}
\hline
\multicolumn{1}{|l|}{}          & \multicolumn{4}{l|}{zero shot}                                                                                            & \multicolumn{4}{l|}{with 1 sample}                                                                                        & \multicolumn{4}{l|}{with 3 sample}                                                                                     \\ \hline
\multicolumn{1}{|l|}{}          & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1}    & \multicolumn{1}{c|}{Accuracy} & \multicolumn{1}{c|}{Precision} & \multicolumn{1}{c|}{Recall} & \multicolumn{1}{c|}{F1} \\ \hline
\multicolumn{13}{|l|}{bloom-3b, "Text:\{text\} What is a possible sentiment for the text given the following options?"}                                                                                                                                                                                                                                                                                          \\ \hline
\multicolumn{1}{|l|}{}          & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & \multicolumn{1}{r|}{44.56} & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & \multicolumn{1}{r|}{44.56} & \multicolumn{1}{r|}{44.56}    & \multicolumn{1}{r|}{19.86}     & \multicolumn{1}{r|}{44.56}  & 44.56                   \\ \hline
\multicolumn{13}{|l|}{bloomz-3b, main method}                                                                                                                                                                                                                                                                                                                                                                    \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{r|}{61.54}    & \multicolumn{1}{r|}{50.83}     & \multicolumn{1}{r|}{61.54}  & \multicolumn{1}{r|}{61.54} & \multicolumn{1}{r|}{58.41}    & \multicolumn{1}{r|}{49.34}     & \multicolumn{1}{r|}{58.41}  & \multicolumn{1}{r|}{58.41} & \multicolumn{1}{r|}{57.83}    & \multicolumn{1}{r|}{48.71}     & \multicolumn{1}{r|}{57.83}  & 57.83                   \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{r|}{61.06}    & \multicolumn{1}{r|}{48.80}     & \multicolumn{1}{r|}{61.06}  & \multicolumn{1}{r|}{61.06} & \multicolumn{1}{r|}{57.80}    & \multicolumn{1}{r|}{50.50}     & \multicolumn{1}{r|}{57.80}  & \multicolumn{1}{r|}{57.80} & \multicolumn{1}{r|}{58.64}    & \multicolumn{1}{r|}{54.89}     & \multicolumn{1}{r|}{58.64}  & 58.64                   \\ \hline
\multicolumn{13}{|l|}{bangla template}                                                                                                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{r|}{58.67}    & \multicolumn{1}{r|}{49.33}     & \multicolumn{1}{r|}{58.67}  & \multicolumn{1}{r|}{58.67} & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       & \multicolumn{1}{r|}{}      & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       &                         \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{r|}{44.94}    & \multicolumn{1}{r|}{55.21}     & \multicolumn{1}{r|}{44.94}  & \multicolumn{1}{r|}{44.94} & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       & \multicolumn{1}{r|}{}      & \multicolumn{1}{r|}{}         & \multicolumn{1}{r|}{}          & \multicolumn{1}{r|}{}       &                         \\ \hline
\multicolumn{13}{|l|}{hindi retrieval dataset}                                                                                                                                                                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|l|}{template0} & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}      & \multicolumn{1}{r|}{53.33}    & \multicolumn{1}{r|}{50.65}     & \multicolumn{1}{r|}{53.33}  & \multicolumn{1}{r|}{53.33} & \multicolumn{1}{r|}{54.30}    & \multicolumn{1}{r|}{50.41}     & \multicolumn{1}{r|}{54.30}  & 54.30                   \\ \hline
\multicolumn{1}{|l|}{template5} & \multicolumn{1}{l|}{}         & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{}      & \multicolumn{1}{r|}{55.47}    & \multicolumn{1}{r|}{46.51}     & \multicolumn{1}{r|}{55.47}  & \multicolumn{1}{r|}{55.47} & \multicolumn{1}{r|}{56.46}    & \multicolumn{1}{r|}{46.88}     & \multicolumn{1}{r|}{56.46}  & 56.46                   \\ \hline
\end{tabular}
\caption{results of two templates in task2 valid of different lines, one bloom-3b, others are bloomz-3b. We use template 0 for "Classify the sentiment of this text as Positive, Negative, or Neutral? \textbackslash{}nText:\{text\}\textbackslash{}nSentiment:", which is used before with english and bengla retrieval dataset. And template 5 for "Text:\{text\} What is a possible sentiment for the text given the following options?", which is used at the end of test.}
\label{tab:results of two templates in task2 valid}
\end{table}



